InstantDrag: Improving Interactivity in Drag-based Image Editing

Drag-based image editing has recently gained popularity for its interactivity and precision. However, despite the ability of text-to-image models to generate samples within a second, drag editing still lags behind due to the challenge of accurately reflecting user interaction while maintaining image content. Some existing approaches rely on computationally intensive per-image optimization or intricate guidance-based methods, requiring additional inputs such as masks for movable regions and text prompts, thereby compromising the interactivity of the editing process. We introduce InstantDrag, an optimization-free pipeline that enhances interactivity and speed, requiring only an image and a drag instruction as input. InstantDrag consists of two carefully designed networks: a drag-conditioned optical flow generator (FlowGen) and an optical flow-conditioned diffusion model (FlowDiffusion). InstantDrag learns motion dynamics for drag-based image editing in real-world video datasets by decomposing the task into motion generation and motion-conditioned image generation. We demonstrate InstantDrag's capability to perform fast, photo-realistic edits without masks or text prompts through experiments on facial video datasets and general scenes. These results highlight the efficiency of our approach in handling drag-based image editing, making it a promising solution for interactive, real-time applications.

==> Figures/figureonly_flowdiffusion.tex <==
\begin{figure*}
    \includegraphics[width=0.8\linewidth]{Materials/figureonly_flowdiffusion.pdf}
    \caption{FlowDiffusion predictions for FlyingChairs datasets.}
    \label{fig:figureonly_flowdiffusion}
\end{figure*}


==> Figures/sup_generalizability_fail.tex <==
\begin{figure*}
    \includegraphics[width=0.95\linewidth]{Materials/Sup_generalizability_fail.pdf}
    \caption{Additional Qualitative Results.}
    \label{fig:sup_generlizability_fail}
\end{figure*}


==> Figures/sup_generalizability_success.tex <==
\begin{figure*}
    \includegraphics[width=0.95\linewidth]{Materials/Sup_generalizability_success.pdf}
    \caption{Additional Qualitative Results.}
    \label{fig:sup_generlizability_success}
\end{figure*}


==> Sections/6_figure_only.tex <==
\input{Figures/ablation}
\input{Figures/figureonly_usingmask}
\input{Figures/figureonly_rginversion}
\input{Figures/figureonly_quali}
\input{Figures/figureonly_flowgen_flowdiffusion}
% \input{Figures/figureonly_flowgen}
%\input{Figures/figureonly_flowdiffusion}
